Using Machine Learning to Optimize Web Interactions on Heterogeneous Mobile Multi-cores

The web has become a ubiquitous application development platform for mobile systems. Yet, web access on mobile devices remains an energy-hungry activity. Prior work in the field mainly focuses on the initial page loading stage, but fails to exploit the opportunities for energy-efficiency optimization while the user is interacting with a loaded page. This paper presents a novel approach for performing energy optimization for interactive mobile web browsing. At the heart of our approach is a set of machine learning models, which estimate \emph{at runtime} the frames per second for a given user interaction input by running the computation-intensive web render engine on a specific processor core under a given clock speed. We use the learned predictive models as a utility function to quickly search for the optimal processor setting to carefully trade responsive time for reduced energy consumption. We integrate our techniques to the open-source Chromium browser and apply it to two representative mobile user events: scrolling and pinching (i.e., zoom in and out). We evaluate the developed system on the landing pages of the top-100 hottest websites and two big.LITTLE heterogeneous mobile platforms. Our extensive experiments show that the proposed approach reduces the system-wide energy consumption by over 36\% on average and up to 70\%. This translates to an over 17\% improvement on energy-efficiency over a state-of-the-art event-based web browser scheduler, but with significantly fewer violations on the quality of service.

==> authors.tex <==

\begin{IEEEbiography}[{\includegraphics[width=1\textwidth]{author/Lu_Yuan.png}}]{Lu Yuan}


was born in 1995. She received her B.S. degree in Computer Science from Northwest University, China, in 2017. She is a master candidate of Computer Science in Northwest University. Her research interests include mobile computing and mobile energy efficiency.

\end{IEEEbiography}




\begin{IEEEbiography}[{\includegraphics[width=1\textwidth]{author/rj.jpg}}]{Jie Ren}


was born in 1988. He received his Ph.D. degree in computer architecture from Northwest University, China, in 2017. He is an assistant professor with the Computer Science Department, Shaanxi Normal University.  His research interests include
mobile computing and performance optimization.
%His address is School of Information Science and Technology, Northwest University, Xi'an, 710127, P.R. China and email address is renjie@nwu.edu.cn.

\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1\textwidth]{author/gl.jpg}}]{Ling Gao}

is currently a professor of computer science at Northwest University, Xi'an, China. He received his BS degree in Computer Science
from Hunan University and his MS degree in Computer Science from Xi'an, Northwest University, in 1985 and 1988 respectively.
In 2005, he received PhD degree in Computer Science from Xi'an Jiaotong University, Xi'an, China.
His research include network security and management, embedded internet service.
\end{IEEEbiography}



\begin{IEEEbiography}[{\includegraphics[width=1\textwidth]{author/Zhanyong_Tang.pdf}}]{Zhanyong Tang}

received his PHD degree in Computer Software and Theory from Northwest University. Now, he is an associate professor in the School of Information Science and Technology, Northwest University. His research interests include network and information security, software security and protection, localization, and wireless sensor network.
\end{IEEEbiography}




\begin{IEEEbiography}[{\includegraphics[width=1\textwidth]{author/alpha.jpg}}]{Zheng Wang}
is an associate professor at the School of Computing at the University of Leeds. His research draws from, combines and contributes to the
areas of compiler-based code optimisation, runtime scheduling, parallel programming and applied machine learning. He is a recipient of the
Best Paper Award in PACT 2010, CGO 2017, PACT 2017 and CGO 2019. He received his PhD from University of Edinburgh in 2011.


\end{IEEEbiography}


==> section/abstract.tex <==
\begin{abstract}

\end{abstract}


==> section/incremental.tex <==
\section{Incremental learning}



==> section/overview.tex <==

\section{Overview of Our Approach}



%Figure~\ref{fig:overview} illustrates the
%workflow of our approach.
%The browser first retrieves the web content,
%and then parses the HTML file to
%identify the embedded objects and styles that the page contains.
%Our extension extracts features to characterize the webpage workload
%during the parsing stage. The off-line trained predictor takes in
%the feature values and outputs a predicted Optimal QoE processor configuration
%$<$\underline{\textbf{{A15-freq}}}, A7-freq$>$.
%Finally, the scheduler which
%is running as a background service,
%configures the processor and schedules the
%rendering process running on the predicted core with a certain frequency.\\
%\textbf{Training Predictor.}
%Figure~\ref{fig:predictive_model}
%depicts the three-stage to train our predictor.
%Training involves extracting feature values and
%finding the best mapping of QoE processor configuration
%for each training webpage, and then feeding these values
%into the SVM machine learning algorithm (see section \ref{sec:modelling}).
%Finally we get the optimal QoE learning a model from the training data.\\
%\textbf{Web Variance.}
%Recent works show that the
%root cause of $webpage$ $variance$ arises
%from the structural (HTML) and
%style (CSS) information\cite{YZhu13},
%and the web contents include different embedded objects to compose
%their structure and styles, such as images, buttons and videos with
%different fonts, colors and sizes.
%The various compositions of web contents contribute to the
%diversity of webpage performance\cite{thiagarajan2012killed}.
%Thus our approach can take
%the advantage of the $webpage$ $variance$
%to schedule the processes to achieve a better user experience
%in heterogeneous multi-processing system.
%
%We develop a Chrome extension to collect features from every webpage,
%and Table~\ref{tab:features} shows the feature details. In the perspective of webpage structure,
%we collect the number of DOM Nodes, depth of DOM Tree and number
%of every HTML tags and attributes. For webpage styles, we collect the number of each
%CSS Properties, CSS Rules and different selector patterns. In addition, we also take
%the webpage size into consideration. Finally, the extension can collect 928 kinds of
%features from every webpage and we will discuss how to deal with them in section \uppercase\expandafter{\romannumeral4}.
%
%
%\begin{figure}
%\begin{center}
%\includegraphics[width=0.5\textwidth]{figure/approach.pdf}
%\end{center}
%\caption{Overview of our approach.}
%\vspace{-6mm}
%\label{fig:overview}
%\end{figure}
%
%\begin{figure}
%\begin{center}
%\includegraphics[width=0.4\textwidth]{figure/predictive_model.pdf}
%\end{center}
%\caption{Predictive model.}
%\vspace{-6mm}
%\label{fig:predictive_model}
%\end{figure}
%
%\begin{table}[b]
%\vspace{-4mm}
%\caption{Features Collection}
%\vspace{-3mm}
%\begin{center}
%\renewcommand{\multirowsetup}{\centering}
%        \begin{tabular}{p{2cm}<{\centering}|p{5cm}<{\centering}}
%        \hline
%        \multirow{4}{2cm}{Structure}
%                & HTML Tags and Count  \\
%                & HTML Attributes and Count\\
%                & DOM Node Count\\
%                & DOM Tree Depth\\
%        \hline
%        \multirow{3}{2cm}{Style}
%                & CSS Properties and Count  \\
%                & CSS Rules Count\\
%                & CSS Selector Patterns and Count\\
%        \hline
%        Others  & Webpage Size\\
%        \hline
%        \end{tabular}
%\end{center}
%\vspace{-5mm}
%\label{tab:features}
%\end{table}








==> section/preamble.tex <==
\usepackage{booktabs}
\usepackage{color, colortbl}
\usepackage{tabularx}
\usepackage{soul}
\usepackage{balance}

\usepackage{graphicx}
\usepackage{subfig}
\usepackage{blindtext}
\usepackage{adjustbox}
\usepackage{multirow}
\usepackage{color}
\usepackage{booktabs}
\usepackage{tabularx}
\usepackage{colortbl}

\usepackage{tikz}
\usepackage{listings}
\usepackage{etoolbox}
\usepackage{subfig}
\usepackage{url}
\usepackage{setspace}
\usepackage[english]{babel}
\usepackage{color, colortbl}
\usepackage{enumitem}
\usepackage{balance}
%\usepackage{hyperref}

\definecolor{Gray}{gray}{0.9}

\newcommand{\circled}[2][]{\tikz[baseline=(char.base)]
	{\node[shape = circle, draw, inner sep = 1pt]
		(char) {\phantom{\ifblank{#1}{#2}{#1}}};%
		\node at (char.center) {\makebox[0pt][c]{#2}};}}
\robustify{\circled}

\newcommand{\ProfileSize}{100MB\xspace}
\newcommand{\PCA}{\texttt{PCA}\xspace}
\newcommand{\cs}{\texttt{cs}\xspace}
\newcommand{\KNN}{\texttt{KNN}\xspace}
\newcommand{\SVM}{\texttt{SVM}\xspace}
\newcommand{\SVMs}{\texttt{SVMs}\xspace}
\newcommand{\NB}{\texttt{NB}\xspace}
\newcommand{\LR}{\texttt{LR}\xspace}
\newcommand{\ANN}{\texttt{ANN}\xspace}
\newcommand{\PCs}{\texttt{PCs}\xspace}
\newcommand{\PC}{\texttt{PC}\xspace}
\newcommand{\RDD}{\texttt{RDD}\xspace}
\newcommand{\RDDs}{\texttt{RDDs}\xspace}
\newcommand{\MLP}{\texttt{MLP}\xspace}

\newcommand{\Quasar}{\textsc{Quasar}\xspace}
\newcommand{\DColocation}{\textsc{Pairwise}\xspace}
\newcommand{\Oracle}{\texttt{oracle}\xspace}
\newcommand{\oracle}{\texttt{oracle}\xspace}
\newcommand\FIXME[1]{\textcolor{red}{FIX:}\textcolor{red}{#1}}

\newcommand{\BBCW}{\texttt{news.bbc.co.uk}\xspace}

\newcommand{\WS}{\texttt{WS}\xspace}
\newcommand{\SML}{\texttt{S-ML}\xspace}

\newcommand{\DOM}{\texttt{DOM}\xspace}

\newcommand{\default}{\texttt{Default}\xspace}
\newcommand{\static}{\texttt{Static}\xspace}
\newcommand{\booster}{\texttt{Booster}\xspace}

\newcommand{\EDP}{\texttt{EDP}\xspace}
\newcommand{\Ondemand}{\texttt{ondemand}\xspace}
\newcommand{\Performance}{\texttt{performance}\xspace}
\newcommand{\Interactive}{\texttt{interactive}\xspace}
\newcommand{\Conservative}{\texttt{conservative}\xspace}
\newcommand{\Powersave}{\texttt{powersave}\xspace}
\newcommand{\bfp}{\texttt{best-performing}\xspace}

\newcommand{\SystemName}{\textsc{Proteus}\xspace}

\newcommand\cparagraph[1]{\vspace{1.5mm} \noindent \textbf{#1}\xspace}
\newcommand\artefactserver{http://124.114.229.91:8888\xspace}
\newcommand\artefactpassword{qscgyjil!@p\xspace}
\newcommand\eg{e.g.,\xspace}
\newcommand\sourcecode{https://github.com/Jiesourcecode/AMBER/}

